AdaNAS: Adaptively Post-processing with Self-supervised Neural Architecture Search for Ensemble Rainfall Forecasts

Previous post-processing studies on rainfall forecasts using numerical weather prediction (NWP) mainly focus on statistics-based aspects, while learning-based aspects are rarely investigated. Although some manually-designed models are proposed to raise accuracy, they are customized networks, which need to be repeatedly tried and verified, at a huge cost in time and labor. Therefore, a self-supervised neural architecture search (NAS) method without significant manual efforts called AdaNAS is proposed in this study to perform rainfall forecast post-processing and predict rainfall with high accuracy. In addition, we design a rainfall-aware search space to significantly improve forecasts for high-rainfall areas. Furthermore, we propose a rainfall-level regularization function to eliminate the effect of noise data during the training. Validation experiments have been performed under the cases of \emph{None}, \emph{Light}, \emph{Moderate}, \emph{Heavy} and \emph{Violent} on a large-scale precipitation benchmark named TIGGE. Finally, the average mean-absolute error (MAE) and average root-mean-square error (RMSE) of the proposed AdaNAS model are 0.98 and 2.04 mm/day, respectively. Additionally, the proposed AdaNAS model is compared with other neural architecture search methods and previous studies. Compared results reveal the satisfactory performance and superiority of the proposed AdaNAS model in terms of precipitation amount prediction and intensity classification. Concretely, the proposed AdaNAS model outperformed previous best-performing manual methods with MAE and RMSE improving by 80.5\% and 80.3\%, respectively.

==> Relatedwork.tex <==
%\vspace{-5mm}
\section{Related work}
%\vspace{-1mm}
\subsection{Precipitation Forecast Post-processing}
%Precipitation prediction is the most critical part of weather forecasting and one of the most difficult tasks. Challenges in precipitation forecasting are complex environments and limitations of atmospheric observations, such as small rain areas, high rain/background similarity and different air masses. In order to maximize the accuracy of rainfall predictions, rainfall predictions typically go through the following process: numerical weather prediction model systems, objective interpretation applications and downscaling gridded post-processing techniques. Among them, the post-processing process is the last step in the refinement of rainfall prediction methods and largely affects the final performance of precipitation prediction.

Precipitation forecast is one of the most difficult tasks in weather forecasting. The challenges in precipitation forecasting include complex environments and limitations of atmospheric observations, such as small rain areas, high rain/background similarity, and different air masses. To increase the accuracy of precipitation forecasts, it typically goes through the following process: NWP model systems, objective interpretation applications and post-processing techniques\cite{dai2016situation}. Among them, the post-processing process is the last step of rainfall prediction methods and largely affects the ultimate performance of precipitation prediction.

%The traditional post-processing process uses simple operations to synthesize the results of ensemble forecasts. The ensemble mean (EM) method averages the results of multiple ensemble forecasts to predict precipitation. The probability matching (PM) method redistributes the precipitation rates in the ensemble mean by the distribution of precipitation rates from the available QPFs\cite{ebert2001ability}. The best percentile (BP) method is a variant of the PM method, which adopts asymmetric normal distribution for parameter estimation to calculate probabilistic quantitative precipitation and percentile forecasts\cite{dai2016situation}. The weighted bias-removed ensemble Mean (WEM) predicts precipitation based on the weighted average of ensemble forecasts, where the weights are calculated from the historical errors of the corresponding models\cite{zhi2011multi}.  Although these methods exhibit different advantages in a variety of test metrics, their precipitation prediction accuracy is still hardly commendable. The latest learning-based approach, which designs a multi-layer network(IC-MLNet)\cite{xu2021multi} to predict precipitation, shows better performance than the various previously mentioned methods in precipitation amount and precipitation levels prediction. It is undoubtedly inefficient to design network architectures manually in order to overcome the precipitation prediction challenges, as evidenced by the long training period of the models and the insignificant improvement of the results. The development of neural architecture search technology has brought hope to solve the precipitation prediction problem.

The traditional post-processing processes use simple operations to synthesize ensemble forecasts. The ensemble mean (EM) method~\cite{kong2006multiresolution} averages multiple ensemble forecasts to predict precipitation. The probability matching (PM) method~\cite{ebert2001ability} redistributes the precipitation rates in the ensemble mean by the distribution of precipitation rates from the available QPFs. The best percentile (BP) method~\cite{dai2016situation} adopts asymmetric normal distribution for parameter estimation to calculate probabilistic quantitative precipitation and percentile forecasts. The weighted bias-removed ensemble mean (WEM)~\cite{zhi2011multi} predicts precipitation based on the weighted average of ensemble forecasts, where the weights are calculated from the historical errors of the ensemble forecasts. Although these methods exhibit different advantages in a variety of test metrics, their precipitation prediction accuracy is still hardly commendable. The reason is that these straightforward methods cannot integrate complex ensemble forecast data.

The latest learning-based approach, which designs a multi-layer network (IC-MLNet)~\cite{xu2021multi} to predict precipitation, shows better performance than traditional methods in precipitation amount and precipitation levels prediction. However, it is undoubtedly inefficient to design network architectures manually to overcome the precipitation prediction challenges, as evidenced by the long training period of models and insignificant improvement of results. The development of neural architecture search technology has brought hope to solve the precipitation prediction problem.

%\vspace{-1mm}
\subsection{Neural Architecture Search}
The neural architecture search (NAS)~\cite{liu2018darts,xu2019pc,he2020milenas,li2021bossnas,ahmed2018maskconnect,you2020greedynas,cai2018proxylessnas,tan2019efficientnet} aims to search for a robust, well-performed neural architecture by automatically selecting and combining different elementary operations from a predefined search space to maximize accuracy for a given task. These NAS-based methods can be divided into three aspects according to the architecture optimization methods~\cite{he2021automl}: (1) evolutionary methods~\cite{ahmed2018maskconnect,you2020greedynas}; (2) reinforcement learning methods~\cite{cai2018proxylessnas,tan2019efficientnet}; (3) gradient descent methods~\cite{liu2018darts,he2020milenas,li2021bossnas,xu2019pc}. The differentiable NAS optimized by the gradient descent method is favored for its fast search speed. Most of the gradient descent-based neural network architecture search methods are dedicated to computer vision research, such as MileNAS~\cite{he2020milenas}, PC-DARTS~\cite{xu2019pc} and BossNAS~\cite{li2021bossnas}. 
%They are all cell-based methods, and such methods usually consist of two levels: one is the cell level~\cite{liu2018darts,xu2019pc}, which selects the operation and connection of nodes in the cell; the other is the network level~\cite{li2021bossnas}, which determines the number of channels and the variation of spatial resolution. However, some approaches~\cite{he2020milenas,xu2019pc} concentrate on the cell level and ignore the network level.Notably, BossNAS exploits contrast learning to implement a self-supervised NAS that works on the network level as well as the cell level.
%Our work is inspired by the self-supervised differentiable NAS~\cite{li2021bossnas} and extends it to a general deterministic precipitation forecast post-processing process.
We design an efficient gradient descent-based  neural architecture search method for rainfall forecast post-processing.

%The neural architecture search (NAS)~\cite{liu2018darts,xu2019pc,he2020milenas,li2021bossnas,ahmed2018maskconnect,you2020greedynas,cai2018proxylessnas,tan2019efficientnet} aims to search for a robust, well-performing neural architecture by automatically selecting and combining different elementary operations from a predefined search space to maximize accuracy for a given task. These NAS-based methods can be divided into four aspects according to architecture optimization methods~\cite{he2021automl}: (1)random methods~\cite{NSAS}; (2) evolutionary methods~\cite{ahmed2018maskconnect,you2020greedynas}; (3) reinforcement learning methods~\cite{cai2018proxylessnas,tan2019efficientnet}; (4) gradient descent methods~\cite{liu2018darts,he2020milenas,li2021bossnas,xu2019pc}. They have their advantages, among which the differentiable NAS optimized by the gradient descent method is favored for its fast search speed. Most of the gradient descent-based neural network architecture search methods are dedicated to computer vision research, such as MileNAS~\cite{he2020milenas}, PC-DARTS~\cite{xu2019pc} and BossNAS~\cite{li2021bossnas}. Our work is inspired by the self-supervised differentiable NAS~\cite{li2021bossnas} and extends it to a general deterministic precipitation forecast post-processing process.

\subsection{Transformer}
Transformer is a module that uses attention mechanisms to improve the accuracy of models, which was first used in natural language processing (NLP) where it achieved significant improvements~\cite{han2022survey,vaswani2017attention,devlin2018bert,brown2020language}. Moreover, transformer-based models that excel not only in NLP but also in computer vision tasks~\cite{chen2020generative,kolesnikov2021image}. The transformer is becoming a potential replacement for convolutional neural network (CNN) or even surpassing CNN. Therefore, we introduce the transformer operation in the search space to improve the accuracy of the high rainfall area.

==> Response.tex <==
\section{Response to Reviewers}
\subsection{To reviewer 1:}
\textbf{Q1: The proposed channel-aware blocks lead to “pixels with significant differences are given a higher weight”. Please explain more about the reason why larger weights on those pixels lead to improvements in forecast accuracy.  }

A: This is because the expressiveness of a small amount of data with important features may be smoothed by a large amount of data with unimportant features or wrong information. Specifically, data characterized by violent storms will show significant differences in certain pixels, but the output of the NWP model (i.e. our input data) may not correctly predict violent storms, which is limited by the accuracy of the NWP model. For example, 20 out of 50 numerical forecasts may be predicted as the storm and the other 30 not. Situations like these can easily soomth the storm forecasts, making the final result generated by the ensemble forecasts, not a storm. Our channel-aware blocks adaptively highlight the importance of features based on their significance, which makes it more difficult for storm forecasts to be smoothed out by other erroneous forecasts, resulting in more accurate storm forecasts.

\textbf{Q2: Why the proposed method performs much better than the previous IC-MLNet? Please add more explanations on which structure in the proposed method leads to the large improvements relative to IC-MLNet in this paper. }

A: We believe that the difference in network structure and module structure has a significant impact on the results. The advantage of network structure can be seen from the TABLE \ref{operation}, which shows that even if we use pure residual block the result is much better than that of IC-MLNet. In addition, the module structure also affects the prediction results; although both our proposed method and IC-MLNet contain convolutional operation blocks, different convolutional block structures have different abilities to abstract data features. It is the difference in network structure and block structure that leads to the huge difference in experimental results. Just like the famous AlexNet and ResNet, although they both consist of convolution layers, the image recognition results are vastly different.

\textbf{Q3: Why multi-model results are worse than single-model results? In my opinion, multi-model predictions usually perform better than single-model results, because multi-model predictions provide more information than single-model results.}

A: It is due to the different numbers of channels of input data in different model modes. In the single-model mode, there are 50 channels of each input data (generated by the same NWP model, under 50 different sets of environmental variables), while in the multi-modal prediction, there are only 4 channels of each input data (generated by 4 different NWP models). Although the multi-model mode contains predictive information from 4 different models, the single-model mode also contains predictive information from NWP models under 50 different environmental variables. In terms of data volume, 50 channels is 12.5 times more than 4 channels and contains more information, so the single-model mode is more effective.

\textbf{Q4: I encourage the code of the proposed algorithm to be released online after the publication of the manuscript to help others learn the algorithm better.}

A: We're sorry, but we can't open-source our code just yet. We will open-source our code later.


\subsection{To reviewer 2:}
\textbf{Q1: Prove that the loss function used is a proper scoring rule.}
%为了证明我们的loss function is a proper scoring rule, 即证明下列不等式：

%其中，E(\dot)表示期望，y表示实际分布，Q表示观测值，P表示预测值，Loss表示损失函数。

%上述不等式可转化为:

%所以只需要证明不等式 A和B

%因为MSE 和HSS为水文模型广泛使用的衡量标准，我们认为没有必要证明他们是否是a proper scoring rule，所以当HSS和MSE loss都符合proper scoring rule的条件时，我们的损失函数也符合proper scoring rule的条件。



A: To prove that our loss function is a proper scoring rule, it is sufficient to prove the following inequality \ref{eq: scoring}:

\begin{equation}
\label{eq: scoring}
E(Loss(Q,y)) \leq E(Loss(P,y))
\end{equation}

where $E(\dot)$ denotes the expectation, y denotes the actual distribution, Q denotes the observed value, P denotes the predicted value and $Loss$ denotes the loss function. The above inequality can be transformed into.

\begin{equation}
\begin{aligned}
\label{eq: scoring2}
E(Loss_{MSE}(Q,y) + \frac{c_H}{loss_{HSS}(Q,y)}) \\
\leq E(Loss_{MSE}(P,y) + \frac{c_H}{loss_{HSS}(P,y)})
\end{aligned}
\end{equation}

So it is only necessary to prove the inequalities \ref{eq: scoring3} and \ref{eq: scoring4}

\begin{equation}
\label{eq: scoring3}
E(Loss_{MSE}(Q,y) \leq E(Loss_{MSE}(P,y) 
\end{equation}

\begin{equation}
\label{eq: scoring4}
E(\frac{c_H}{loss_{HSS}(Q,y)}) \leq E(\frac{c_H}{loss_{HSS}(P,y)})
\end{equation}

Because MSE and HSS are widely used measures for hydrological models, we do not think it is necessary to prove whether they are proper scoring rules or not, so when both HSS and MSE loss functions qualify as proper scoring rules, our loss functions also qualify as proper scoring rules.

\textbf{Q2: Add a few benchmark methods that are criticized for being time-consuming etc. and cross-compare the performances and test if the differences are statistically significant, then adjust the Diebold-Mariano test results for the effects of test multiplicity (simultaneously analyzing multiple hypothesis test results) by controlling the false discovery rate.}
%我们在实验小节增加了四个方法的验证时间测试。此外，我们还新增了Diebold-Mariano test。我们认为multiple hypothesis test不是很有必要。一方面是因为我们已经有acc和hss两个分类指标，另一方面，multiple hypothesis test主要用于验证小概率错误事件，就现在的降雨分类准确度而言，没有必要使用multiple hypothesis test。

A: We have added a test on validation time consumption to Section \ref{sec: time}. In addition, in Section \ref{sec: PAP}, we added the Diebold-Mariano test to show that our method is statistically superior to other methods, that's why we consider that the multiple hypothesis test is probably unnecessary. On the one hand, it is because we already have two classification metrics, ACC and HSS, and on the other hand, the multiple hypothesis tests are mainly used to validate small probability of error events, and it is not necessary to use the multiple hypothesis tests in view of the current accuracy of rainfall classification.
